Ergodic Fading One-sided Interference Channels without State Information at Transmitters

This work studies the capacity region of a two-user ergodic interference channel with fading, where only one of the users is subject to interference from the other user, and the channel state information (CSI) is only available at the receivers. A layered erasure model with one-sided interference and with arbitrary fading statistics is studied first, whose capacity region is completely determined as a polygon. Each dominant rate pair can be regarded as the outcome of a trade-off between the rate gain of the interference-free user and the rate loss of the other user due to interference. Using insights from the layered erasure model, inner and outer bounds of the capacity region are provided for the one-sided fading Gaussian interference channels. In particular, the inner bound is achieved by artificially creating layers in the signaling of the interference-free user. The outer bound is developed by characterizing a similar trade-off as in the erasure model by taking a "layered" view using the incremental channel approach. Furthermore, the gap between the inner and outer bounds is no more than 12.772 bits per channel use per user, regardless of the signal-to-noise ratios and fading statistics.

==> figs/figCap.tex <==
\begin{tikzpicture}
        \coordinate (origin) at (0, 0);
      \draw[->, ultra thick] (0,0) -- (6,0) node[below] {$R_1$};
        \draw[->, ultra thick] (0,0) -- (0, 8.5) node[left] {$R_2$};
        \coordinate (C1) at (4,0);
        \coordinate (C11) at (4,10);
        \coordinate (C2) at (0,6);
        \coordinate (C22) at (10,6);
        % points on lines
        \coordinate (L1x) at (4.5,0);
        \coordinate (L1y) at (0,13.5);
        \coordinate (L2x) at (5,0);
        \coordinate (L2y) at (0,10);
        \coordinate (L3x) at (5.8,0);
        \coordinate (L3y) at (0,8.7);
        \coordinate (L4x) at (8,0);
        \coordinate (L4y) at (0,8);
        % cross points
        \coordinate (L0) at (intersection of C1--C11 and L1x--L1y);
        \coordinate (L1) at (intersection of L1x--L1y and L2x--L2y);
        \coordinate (L2) at (intersection of L2x--L2y and L3x--L3y);
        \coordinate (L3) at (intersection of L3x--L3y and L4x--L4y);
        
        %draw segments
        \draw[very thick] (C1) node [below]{\small $\MEXP \rN_{1}$}--(L0);
        \draw[very thick] (L0) --node[above, sloped]{$\omega_1$} (L1);
        \draw[very thick] (L1)node[right]{$L_1$} --node[above, sloped]{$\omega_2$} (L2)node[right]{$L_2$};
        \coordinate (up) at (intersection of C2--C22 and L2--L3);
        \draw[very thick] (C2) node[left]{\small$\MEXP \rN_{2}$}--(up);
        \draw[very thick] (up)--(L2);
        \draw[very thick] (L3)node[right]{$L_3$} --node[above, sloped]{$1$} (L4y);
        \draw[very thick] (L3) -- node[above, sloped]{$\omega_3$}(L2);
        \fill[black] (C1) circle (1mm);
        \fill[black] (C2) circle (1mm);
        \node[star, inner sep=.6mm,draw=red, fill=red] at (L0) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (up) {};
       \node[star, inner sep=.6mm,draw=red, fill=red] at (L1) {};
        \node[star, inner sep=.6mm,draw=red, fill=red] at (L2) {};
        \node[star, inner sep=.6mm,draw=red, fill=red] at (L3) {};
        \draw[very thick, dashed] (L0) node[right]{$L_0$}--( L0 -| C2) node[left]{\small $\MEXP \left[\rN_{0}
            - \rN_{1} \right]^+$};
        \draw[->, thick] (4.5,6) node[anchor=south west]{Curve $\setL$}--(2.5,5.5);
        \draw[->, thick] (5.5,6) -- (4.3, 2.8);
\end{tikzpicture}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figGauOuter.tex <==
\begin{tikzpicture}
        \coordinate (origin) at (0, 0);
      \draw[->, ultra thick] (0,0) -- (8.5,0) node[below] {$R_1$};
        \draw[->, ultra thick] (0,0) -- (0, 8.5) node[left] {$R_2$};
        \coordinate (C1) at (5,0);
        \coordinate (C11) at (5,1.5);
        \coordinate (C2) at (0,6.5);
        \coordinate (C22) at (10,6.5);
        \coordinate (cor) at (1,6);
        \draw  (C1) -- (C11);
        \draw (C11) -- (cor);
\end{tikzpicture}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figQ1Ach1.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,1);
        \coordinate  (r_33) at (10,1);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \coordinate (c) at (intersection of r_3--r_33 and r_1--r_11);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[dashed] (a_1) -- (a_2);
        % \draw[dashed] (a) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11); 
        %\draw (a) -- (b);
        \draw[dashed] (b)--(c);
        \draw[very thick] (c)--(r_1) node[below]{\small$\Ces_{1}$};
        % \draw[dashed] (b)--(a_1);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_{1}$};
        \draw[dashed] (a)--(1.5,0) node[below]{\small $\Ces_{1}\epsilon_{0}$};
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        \draw [->] (3.3,3.3) node[above] {\small$\tiny R_1 + R_2 = 1-\epsilon_0 \epsilon_1$}--(2.4,2.4);
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../Z_RCSI"
%%% End: 


==> figs/figQ1Ach2.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,2.5);
        \coordinate  (r_33) at (10,2.5);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \draw[dashed] (a_1) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11);
        \coordinate (e) at (1.5,0);
        \coordinate (d) at (intersection of a--e and origin--a_1);
        \draw[very thick] (b)--(r_1) node[below]{\small $\Ces_{1}$};
        \draw[dashed] (a)--(d)node[below]{\small$\Ces_{1}\epsilon_0$};
        \coordinate (c) at (intersection of r_3--r_33 and a_1--a_2);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[very thick] (c)--(b);
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        %\fill[red] (c) circle (1mm);
        \node[star, inner sep=.6mm,draw=red, fill=red] at (c) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (b) {};
        \draw [->] (3.3,3.3) node[above] {\small$\tiny R_1 + R_2 = 1-\epsilon_0 \epsilon_1$}--(2.4,2.4);
        \coordinate (f) at (0,1.5);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_1$};
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Z_RCSI"
%%% End: 


==> figs/figQ1Ach3.tex <==
    \begin{tikzpicture}[scale=.8]
        \draw [<->,ultra thick] (0,5) node (yaxis) [above] {$R_2$}
        |- (5,0) node (xaxis) [right] {$R_1$};
        \coordinate (origin) at (0,0);
        \coordinate  (r_2) at (0,3);
        \coordinate  (r_22) at (10,3);
        \coordinate  (r_1) at (3,0);
        \coordinate  (r_11) at (3,10);
        \coordinate  (r_3) at (0,3.5);
        \coordinate  (r_33) at (10,3.5);
        \coordinate  (a_2) at (0,4.5);
        \coordinate  (a_1) at (4.5,0);
        \coordinate (a) at (intersection of r_2--r_22 and a_1--a_2);
        \draw[dashed] (r_2) node[left]{$\Ces_{0}$}-- (a);
        \draw[dashed] (a_1) -- (a_2);
        \coordinate (b) at (intersection of a_1--a_2 and r_1--r_11);
        \coordinate (e) at (1.5,0);
        \coordinate (d) at (intersection of a--e and origin--a_1);
        \draw[very thick] (b)--(r_1) node[below]{\small $\Ces_{1}$};
        \draw[dashed] (a)--(d)node[below]{\small$\Ces_{1}\epsilon_0$};
        \coordinate (c) at (intersection of r_3--r_33 and a--e);
        \draw[very thick] (r_3) node[left]{$\Ces_{2}$}--(c);
        \draw[very thick] (c)--(b);
        \draw[dashed] (a)--(c);
        \fill[black] (r_2) circle (1mm);
        \fill[black] (r_1) circle (1mm);
        \node[star, inner sep=.6mm,draw=red, fill=red] at (c) {};
        \node[rectangle, inner sep=1mm,draw=blue, fill=blue] at (b) {};
        \draw [->] (3.5,4) node[above] {\small$\tiny R_1 + R_2 = 1-\epsilon_0 \epsilon_1$}--(1.8,2.8);
      \coordinate (f) at (0,1.5);
        \draw[dashed] (b)--(0,1.5) node[left]{\small $\Ces_{0}\epsilon_{1}$};
        \fill[nearly transparent, green!70!white] (r_2)--(a)--(b)--(r_1)--(origin)--cycle;
      \end{tikzpicture}


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Z_RCSI"
%%% End: 


==> zycommandset.tex <==
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defi}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}

\newcommand{\mbA}{\mathbf{A}}
\newcommand{\mbB}{\mathbf{B}}
\newcommand{\mbC}{\mathbf{C}}
\newcommand{\mbD}{\mathbf{D}}
\newcommand{\mbE}{\mathbf{E}}
\newcommand{\mbF}{\mathbf{F}}
\newcommand{\mbG}{\mathbf{G}}
\newcommand{\mbH}{\mathbf{H}}
\newcommand{\mbI}{\mathbf{I}}
\newcommand{\mbJ}{\mathbf{J}}
\newcommand{\mbK}{\mathbf{K}}
\newcommand{\mbL}{\mathbf{L}}
\newcommand{\mbM}{\mathbf{M}}
\newcommand{\mbN}{\mathbf{N}}
\newcommand{\mbO}{\mathbf{O}}
\newcommand{\mbP}{\mathbf{P}}
\newcommand{\mbQ}{\mathbf{Q}}
\newcommand{\mbR}{\mathbf{R}}
\newcommand{\mbS}{\mathbf{S}}
\newcommand{\mbT}{\mathbf{T}}
\newcommand{\mbU}{\mathbf{U}}
\newcommand{\mbV}{\mathbf{V}}
\newcommand{\mbW}{\mathbf{W}}
\newcommand{\mbX}{\mathbf{X}}
\newcommand{\mbY}{\mathbf{Y}}
\newcommand{\mbZ}{\mathbf{Z}}

\newcommand{\mba}{\mathbf{a}}
\newcommand{\mbb}{\mathbf{b}}
\newcommand{\mbc}{\mathbf{c}}
\newcommand{\mbd}{\mathbf{d}}
\newcommand{\mbe}{\mathbf{e}}
\newcommand{\mbf}{\mathbf{f}}
\newcommand{\mbg}{\mathbf{g}}
\newcommand{\mbh}{\mathbf{h}}
\newcommand{\mbi}{\mathbf{i}}
\newcommand{\mbj}{\mathbf{j}}
\newcommand{\mbk}{\mathbf{k}}
\newcommand{\mbl}{\mathbf{l}}
\newcommand{\mbm}{\mathbf{m}}
\newcommand{\mbn}{\mathbf{n}}
\newcommand{\mbo}{\mathbf{o}}
\newcommand{\mbp}{\mathbf{p}}
\newcommand{\mbq}{\mathbf{q}}
\newcommand{\mbr}{\mathbf{r}}
\newcommand{\mbs}{\mathbf{s}}
\newcommand{\mbt}{\mathbf{t}}
\newcommand{\mbu}{\mathbf{u}}
\newcommand{\mbv}{\mathbf{v}}
\newcommand{\mbw}{\mathbf{w}}
\newcommand{\mbx}{\mathbf{x}}
\newcommand{\mby}{\mathbf{y}}
\newcommand{\mbz}{\mathbf{z}}

\newcommand{\ud}{\mathrm{d}}
\newcommand{\uT}{\mathrm{T}}
\newcommand{\uH}{\mathrm{H}}


\newcommand{\fixme}[1]{{\color{red} #1}}
\newcommand{\modify}[1]{{\color{blue} #1}}
\newcommand{\comment}[1]{{\color{green} #1}}

==> zymacroset.tex <==
\usepackage{ifthen}

\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{coro}[theorem]{Corollary}
\newtheorem{defn}{Definition}
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}
\newtheorem{example}{Example}
\newtheorem{conj}{Conjecture}
\newtheorem{claim}{Claim}

\ifthenelse{\equal{\dongningstyle}{true}}{
        \newcommand{\RVEC}[1]{\boldsymbol{\uppercase{#1}}}
        \newcommand{\RMAT}[1]{\underline{\boldsymbol{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\uppercase{#1}}
        \newcommand{\VEC}[1]{\boldsymbol{\lowercase{#1}}}
        \newcommand{\MAT}[1]{\boldsymbol{\underline{\lowercase{#1}}}}
}{
        \newcommand{\RVEC}[1]{\boldsymbol{#1}}
        \newcommand{\RMAT}[1]{\boldsymbol{\mathrm{\uppercase{#1}}}}
        \newcommand{\RSCA}[1]{\boldsymbol{#1}}
        \newcommand{\VEC}[1]{#1}
        \newcommand{\MAT}[1]{\mathrm{\uppercase{#1}}}
}




\newcommand{\snr}{\mathsf{snr}}
\newcommand{\mmse}[1]{\mathsf{mmse}\left[ #1 \right]}
\newcommand{\inr}{\mathsf{INR}}
\newcommand{\MEXP}{\mathbb{E}}
\newcommand{\Prob}[1]{\mathsf{P}\left( #1 \right)}
\newcommand{\Probb}{\mathsf{P}}
\newcommand{\LOG}[1]{\log \left( #1 \right)}
\newcommand{\HAT}[1]{\widehat{#1}}
\newcommand{\TIT}[1]{\widetilde{#1}}
\newcommand{\FLR}[1]{\lfloor #1 \rfloor}
%\allowdisplaybreaks

\newcommand{\uT}{\mathsf{T}}
\newcommand{\ud}{\mathsf{d}}
\newcommand{\trace}{\mathsf{tr}}


\newcommand{\fixme}[1]{{\color{Orangered} #1}}
\newcommand{\modify}[1]{{\color{Navyblue} #1}}

\newcommand{\IE}{{\it i.e.}}

